Experimental systematic uncertainties (and object reconstruction) on top physics, their correlations, comparison ATLAS vs CMS (vs Tevatron) and common agreements

The experimental systematic uncertainties associated to the reconstruction and calibration of the objects appearing in top quark final states at the LHC and Tevatron are discussed. The strategies followed in the ATLAS and CMS experiments are compared in detail for the cases of the jet energy scale and $b$-tagging calibrations, where a categorisation of the associated uncertainty sources as well as the corresponding correlations across experiments has been proposed. The estimate of the non-prompt and fake lepton background to the top quark leptonic channels is also discussed.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = ExperimentalSystematics_MJCosta

default: testpdflatex

testlatex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}
	

testpdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg \
              *.inx *.dvi *.toc *.out *~ ~* */*~ */~* spellTmp 

